QDiff: Differential Testing of Quantum Software Stacks

Over the past few years, several quantum software stacks (QSS) have been developed in response to rapid hardware advances in quantum computing. A QSS includes a quantum programming language, an optimizing compiler that translates a quantum algorithm written in a high-level language into quantum gate instructions, a quantum simulator that emulates these instructions on a classical device, and a software controller that sends analog signals to a very expensive quantum hardware based on quantum circuits. In comparison to traditional compilers and architecture simulators, QSSes are difficult to tests due to the probabilistic nature of results, the lack of clear hardware specifications, and quantum programming complexity. This work devises a novel differential testing approach for QSSes, named QDIFF with three major innovations: (1) We generate input programs to be tested via semantics-preserving, source to source transformation to explore program variants. (2) We speed up differential testing by filtering out quantum circuits that are not worthwhile to execute on quantum hardware by analyzing static characteristics such as a circuit depth, 2 qubit gate operations, gate error rates, and T1 relaxation time. (3) We design an extensible equivalence checking mechanism via distribution comparison functions such as Kolmogorov Smirnov test and cross entropy

==> code/MotivationOriginalCircuit.tex <==
\begin{quantikz}[row sep={0.8cm,between origins}]
%\lstick{\ket{0}} & \phase{\alpha} & \gate{H} & \phase{\beta} & \gate{H} & \phase{\gamma} & \meter{$\ket{\pm}$} \\
& \ctrl{2} & \qw & \gate{X} & \ctrl{1} & \qw \\
& \qw & \ctrl{2} & \gate{X} & \gate{Z^{0.1}} & \qw \\
& \gate{Z^{0.1}} & \qw & \gate{X} & \ctrl{1} & \qw \\
& \qw & \gate{Z^{0.1}} & \gate{X} & \gate{Z^{0.1}} & \qw \\
\end{quantikz}

==> code/MotivationTransformedCircuit.tex <==
\begin{quantikz}[row sep={0.8cm,between origins}]
%\lstick{\ket{0}} & \phase{\alpha} & \gate{H} & \phase{\beta} & \gate{H} & \phase{\gamma} & \meter{$\ket{\pm}$} \\
& \ctrl{2} & \qw & \gate{X} & \ctrl{1} & \qw \\
& \qw & \ctrl{2} & \gate{X} & \gate{Z^{2.1}} & \qw \\
& \gate{Z^{2.1}} & \qw & \gate{X} & \ctrl{1} & \qw \\
& \qw & \gate{Z^{2.1}} & \gate{X} & \gate{Z^{2.1}} & \qw \\
\end{quantikz}

==> code/circuit.tex <==
\begin{quantikz}[column sep = 0.5cm,row sep={0.8cm,between origins}]
%\lstick{\ket{0}} & \phase{\alpha} & \gate{H} & \phase{\beta} & \gate{H} & \phase{\gamma} & \meter{$\ket{\pm}$} \\
\lstick{\#(0,0)} & \gate{X^\alpha} & \qw & \ctrl{2}\gategroup[wires=3,steps=1,style={dashed,
rounded corners,fill=blue!20,inner xsep=0.5pt,inner sep=0.1pt},background]{$CZ^\gamma$} & \qw & \gate{X} & \ctrl{1}\gategroup[wires=2,steps=1,style={dashed,
rounded corners,fill=blue!20,inner xsep=0.5pt,inner sep=0.1pt},background]{$CZ^\gamma$} & \gate{X} & \meter{} \\
\lstick{\#(0,1)} & \gate{X^\alpha} & \gate{Z^\beta} & \qw & \ctrl{2}\gategroup[wires=3,steps=1,style={dashed,
rounded corners,fill=blue!20,inner xsep=0.5pt,inner sep=0.1pt},background,label style={label position=below,anchor=
north,yshift=-0.1cm}]{$CZ^\gamma$} & \gate{X} & \gate{Z^\gamma} & \gate{X} & \meter{} \\
\lstick{\#(1,0)} & \gate{X^\alpha} & \qw & \gate{Z^\gamma} & \qw & \gate{X} & \ctrl{1}\gategroup[wires=2,steps=1,style={dashed,
rounded corners,fill=blue!20,inner xsep=0.5pt,inner sep=0.1pt},background,label style={label position=below,anchor=
north,yshift=-0.1cm}]{$CZ^\gamma$} & \gate{X} & \meter{} \\
\lstick{\#(1,1)} & \gate{X^\alpha} & \gate{Z^\beta} & \qw & \gate{Z^\gamma} & \gate{X} & \gate{Z^\gamma} & \gate{X} & \meter{} 
\end{quantikz}

==> code/evaluation_cirq_1.tex <==
\lstset{language=Python}
\begin{lstlisting}[style=MyCSmallStyle]
return cirq.PointOptimizationSummary(clear_span=1,
    clear_qubits=(cirq.GridQubit(1,2),cirq.GridQubit(2,3)),
    new_operations=[
        cirq.CZ(*op.qubits),
        cirq.X.on_each(*op.qubits),
        cirq.X.on_each(*op.qubits)])
\end{lstlisting}

==> code/evaluation_cirq_2.tex <==
\lstset{language=Python}
\begin{lstlisting}[style=MyCSmallStyle]
return cirq.PointOptimizationSummary(clear_span=-1,
    clear_qubits=*op.qubits,
    new_operations=[
        cirq.CZ(*op.qubits),
        cirq.X.on_each(*op.qubits),
        cirq.X.on_each(*op.qubits)])
\end{lstlisting}

==> code/evaluation_qiskit_3.tex <==
\lstset{language=Python}
\begin{lstlisting}[style=MyCSmallStyle]
    input_qubit = QuantumRegister(n,"qc")
    classical = ClassicalRegister(n, "qm")
    prog = QuantumCircuit(input_qubit, classical)
    prog.cnot(0,1)
    prog.cnot(1,0)
    prog.cnot(0,1)
\end{lstlisting}

==> code/motivate_example_cirq.tex <==
\lstset{language=Python}
\begin{lstlisting}[style=MyCSmallStyle]
    import sympy
    circuit = cirq.Circuit()
    alpha = sympy.Symbol('alpha')
    beta = sympy.Symbol('beta')
    gamma = sympy.Symbol('gamma')
    circuit.append(one_step(h, jr, jc, alpha, beta, gamma))
    circuit.append(cirq.measure(*qubits, key='x'))
    print(circuit)
    print(simulator.run(circuit,repetitions=1024))
\end{lstlisting}

==> code/motivate_example_pyquil.tex <==
\lstset{language=Python}
\begin{lstlisting}[style=MyCSmallStyle]
    qvm = get_qc('3q-qvm')
    try:
        qvm.run(Program())
    except:
        print("empty")
    qvm.run(Program(H(1)))
\end{lstlisting}


==> code/toolong_circuit.tex <==
\begin{quantikz}[column sep = 0.5cm,row sep=0.1cm,between origins]
%\lstick{\ket{0}} & \phase{\alpha} & \gate{H} & \phase{\beta} & \gate{H} & \phase{\gamma} & \meter{$\ket{\pm}$} \\
\lstick{l0--\#qc0} &\ctrl{1} & \gate[4,style={rectangle,fill=white,draw=black,line width=1pt,inner xsep=0pt,inner ysep=0pt}]{\text{79 moments}}  &\qw &\qw \\
\lstick{l1--\#qc1} &\gate{X} &\qw  &\gate{\sqrt{X}}&\qw \\
\lstick{l2--\#qc3}  &\gate{Rz(pi/2)} &\qw &\ctrl{1} &\qw\\
\lstick{l3--\#qc4} &\qw & \qw &\gate{X} &\qw\\
\end{quantikz}

==> table/different_circuit_depth.tex <==



\pgfplotsset{
    box plot/.style={
        /pgfplots/.cd,
        black,
        only marks,
        mark=-,
        mark size=\pgfkeysvalueof{/pgfplots/box plot width},
        /pgfplots/error bars/y dir=plus,
        /pgfplots/error bars/y explicit,
        /pgfplots/table/x index=\pgfkeysvalueof{/pgfplots/box plot x index},
    },
    box plot box/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \draw  ##1 -- ++(\pgfkeysvalueof{/pgfplots/box plot width},0pt) |- ##2 -- ++(-\pgfkeysvalueof{/pgfplots/box plot width},0pt) |- ##1 -- cycle;
        },
        /pgfplots/table/.cd,
        y index=\pgfkeysvalueof{/pgfplots/box plot box top index},
        y error expr={
            \thisrowno{\pgfkeysvalueof{/pgfplots/box plot box bottom index}}
            - \thisrowno{\pgfkeysvalueof{/pgfplots/box plot box top index}}
        },
        /pgfplots/box plot
    },
    box plot top whisker/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark}%
            {\pgfplotserrorbarsmark}%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark options}%
            {\pgfplotserrorbarsmarkopts}%
            \path ##1 -- ##2;
        },
        /pgfplots/table/.cd,
        y index=\pgfkeysvalueof{/pgfplots/box plot whisker top index},
        y error expr={
            \thisrowno{\pgfkeysvalueof{/pgfplots/box plot box top index}}
            - \thisrowno{\pgfkeysvalueof{/pgfplots/box plot whisker top index}}
        },
        /pgfplots/box plot
    },
    box plot bottom whisker/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark}%
            {\pgfplotserrorbarsmark}%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark options}%
            {\pgfplotserrorbarsmarkopts}%
            \path ##1 -- ##2;
        },
        /pgfplots/table/.cd,
        y index=\pgfkeysvalueof{/pgfplots/box plot whisker bottom index},
        y error expr={
            \thisrowno{\pgfkeysvalueof{/pgfplots/box plot box bottom index}}
            - \thisrowno{\pgfkeysvalueof{/pgfplots/box plot whisker bottom index}}
        },
        /pgfplots/box plot
    },
    box plot median/.style={
        /pgfplots/box plot,
        /pgfplots/table/y index=\pgfkeysvalueof{/pgfplots/box plot median index}
    },
    box plot width/.initial=1em,
    box plot x index/.initial=0,
    box plot median index/.initial=1,
    box plot box top index/.initial=2,
    box plot box bottom index/.initial=3,
    box plot whisker top index/.initial=4,
    box plot whisker bottom index/.initial=5,
}

\newcommand{\boxplot}[2][]{
    \addplot [box plot median,#1] table {#2};
    \addplot [forget plot, box plot box,#1] table {#2};
    \addplot [forget plot, box plot top whisker,#1] table {#2};
    \addplot [forget plot, box plot bottom whisker,#1] table {#2};
}


\begin{tikzpicture}
\begin{axis} [symbolic x coords={P1,P2,P3,P4,P5,P6,P7},
ylabel = {$\Delta$ of Circuit Depth},
	  ylabel near ticks,
box plot width=2mm]
\boxplot [
    forget plot,
    box plot x index=0,
    box plot whisker bottom index=1,
    box plot whisker top index=5,
    box plot box bottom index=2,
    box plot box top index=4,
    box plot median index=3
] {testdata.dat}

\end{axis}
\end{tikzpicture}

==> table/different_gate.tex <==



\pgfplotsset{
    box plot/.style={
        /pgfplots/.cd,
        black,
        only marks,
        mark=-,
        mark size=\pgfkeysvalueof{/pgfplots/box plot width},
        /pgfplots/error bars/y dir=plus,
        /pgfplots/error bars/y explicit,
        /pgfplots/table/x index=\pgfkeysvalueof{/pgfplots/box plot x index},
    },
    box plot box/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \draw  ##1 -- ++(\pgfkeysvalueof{/pgfplots/box plot width},0pt) |- ##2 -- ++(-\pgfkeysvalueof{/pgfplots/box plot width},0pt) |- ##1 -- cycle;
        },
        /pgfplots/table/.cd,
        y index=\pgfkeysvalueof{/pgfplots/box plot box top index},
        y error expr={
            \thisrowno{\pgfkeysvalueof{/pgfplots/box plot box bottom index}}
            - \thisrowno{\pgfkeysvalueof{/pgfplots/box plot box top index}}
        },
        /pgfplots/box plot
    },
    box plot top whisker/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark}%
            {\pgfplotserrorbarsmark}%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark options}%
            {\pgfplotserrorbarsmarkopts}%
            \path ##1 -- ##2;
        },
        /pgfplots/table/.cd,
        y index=\pgfkeysvalueof{/pgfplots/box plot whisker top index},
        y error expr={
            \thisrowno{\pgfkeysvalueof{/pgfplots/box plot box top index}}
            - \thisrowno{\pgfkeysvalueof{/pgfplots/box plot whisker top index}}
        },
        /pgfplots/box plot
    },
    box plot bottom whisker/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark}%
            {\pgfplotserrorbarsmark}%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark options}%
            {\pgfplotserrorbarsmarkopts}%
            \path ##1 -- ##2;
        },
        /pgfplots/table/.cd,
        y index=\pgfkeysvalueof{/pgfplots/box plot whisker bottom index},
        y error expr={
            \thisrowno{\pgfkeysvalueof{/pgfplots/box plot box bottom index}}
            - \thisrowno{\pgfkeysvalueof{/pgfplots/box plot whisker bottom index}}
        },
        /pgfplots/box plot
    },
    box plot median/.style={
        /pgfplots/box plot,
        /pgfplots/table/y index=\pgfkeysvalueof{/pgfplots/box plot median index}
    },
    box plot width/.initial=1em,
    box plot x index/.initial=0,
    box plot median index/.initial=1,
    box plot box top index/.initial=2,
    box plot box bottom index/.initial=3,
    box plot whisker top index/.initial=4,
    box plot whisker bottom index/.initial=5,
}

\newcommand{\boxplot}[2][]{
    \addplot [box plot median,#1] table {#2};
    \addplot [forget plot, box plot box,#1] table {#2};
    \addplot [forget plot, box plot top whisker,#1] table {#2};
    \addplot [forget plot, box plot bottom whisker,#1] table {#2};
}


\begin{tikzpicture}
\begin{axis} [
symbolic x coords={P1,P2,P3,P4,P5,P6,P7},
 ylabel = {$\Delta$ of 2-qubit gate},
	  ylabel near ticks,
box plot width=2mm]
\boxplot [
    forget plot,
    box plot x index=0,
    box plot whisker bottom index=1,
    box plot whisker top index=5,
    box plot box bottom index=2,
    box plot box top index=4,
    box plot median index=3
] {testdata2.dat}

\end{axis}
\end{tikzpicture}
